$O(\log^2k/\log\log{k})$-Approximation Algorithm for Directed Steiner Tree: A Tight Quasi-Polynomial-Time Algorithm

In the Directed Steiner Tree (DST) problem we are given an $n$-vertex directed edge-weighted graph, a root $r$, and a collection of $k$ terminal nodes. Our goal is to find a minimum-cost arborescence that contains a directed path from $r$ to every terminal. We present an $O(\log^2 k/\log\log{k})$-approximation algorithm for DST that runs in quasi-polynomial-time. By adjusting the parameters in the hardness result of Halperin and Krauthgamer, we show the matching lower bound of $\Omega(\log^2{k}/\log\log{k})$ for the class of quasi-polynomial-time algorithms. This is the first improvement on the DST problem since the classical quasi-polynomial-time $O(\log^3 k)$ approximation algorithm by Charikar et al. (The paper erroneously claims an $O(\log^2k)$ approximation due to a mistake in prior work.) Our approach is based on two main ingredients. First, we derive an approximation preserving reduction to the Label-Consistent Subtree (LCST) problem. The LCST instance has quasi-polynomial size and logarithmic height. We remark that, in contrast, Zelikovsky's heigh-reduction theorem used in all prior work on DST achieves a reduction to a tree instance of the related Group Steiner Tree (GST) problem of similar height, however losing a logarithmic factor in the approximation ratio. Our second ingredient is an LP-rounding algorithm to approximately solve LCST instances, which is inspired by the framework developed by Rothvo{\ss}. We consider a Sherali-Adams lifting of a proper LP relaxation of LCST. Our rounding algorithm proceeds level by level from the root to the leaves, rounding and conditioning each time on a proper subset of label variables. A small enough (namely, polylogarithmic) number of Sherali-Adams lifting levels is sufficient to condition up to the leaves.

==> overview.tex <==
\section{Overview and Inituition of the Algorithms}
\label{sec:overview}

\bur{There is some repetition with the introduction, but I want just to make the readers get some key ideas (by repeating the same information), enough to re-construct the proofs if necessary.}
This section provides a big picture overview of our key idea and algorithms. While we do not expect a deep background on Sherali-Adams lifting techniques, we assume a small knowledge of basic data structure algorithms. 

\subsection{The First Ingredient: Replacing the Height-Reduction theorem}
\label{sec:overview:height-reduction}

Firstly, as we have mentioned all of the algorithms for DST \cite{CharikarCCDGGL99,ZosinK02,Rothvoss11,FriggstadKKLST14} require a prerequisite that there exists a considerably {\bf cheap} solution that is an out-arborescence with {\bf small height}. Let us say there exists an arborescence $T$ with height $h$ whose cost is at most $f(h)$ times the optimum. To meet the criteria, they rely on the Zelikovsky's Height-Reduction theorem \cite{Zelikovsky97,HelvigRZ01}, which shows an existence of an out-arborescence of height $h$ with $f(h)=h{k}^{1/h}$, where $k$ is the number of leaves of $T$, and such a solution exists in the metric-closure of the input graph.
To obtain an improvement, one require developing a new Height-Reduction theorem that incurs no (or small) factor loss in an approximation ratio. There has been an attempt to improve the theorem \cite{ChekuriEGXXXX}; however, their result requires the input graph to be a tree.
%

Nevertheless, for undirected graph, there exists a Height Reduction that incurs no factor loss, and this is, in fact, a standard Data Structure technique that has been taught in the undergraduate level courses.
% 
To illustrate, let us consider an undirected binary tree $T$ rooted at $r$ with $n$ vertices and $k$ leaves, but its height can be arbitrary. (Perhaps, the readers may think of $T$ as a very unbalanced binary search tree.)
From a standard Data-Structure textbook, we know that $T$ can be made balanced or even a perfect binary tree by using rotation technique. In particular, we find a vertex $v$ that separates $T$ into roughly two equal-size subtrees, say $T_{left}$ and $T_{right}$, where each subtree has size at most $2n/3$. Then we can rotate $T$ around the vertex $v$ so that $v$ becomes the root, and $T_{left}$ and $T_{right}$ become left and right subtrees of the new tree, respectively.
This reduces the height of the tree $T$ by at least one; however, it might not yet be balanced because $T_{left}$ or $T_{right}$ may have height larger than $\log_{2/3}{2n/3}$.
Somehow, we can apply the operation recursively on $T_{left}$ and $T_{right}$ until we obtain a tree ${\bf T}$ of height $O(\log n)$ (and thus is a balanced binary tree).
(Note that the root of each subtree $T_{left}$ and $T_{right}$ will be modified during the recursion.)
It can be seen that this operation gives us a tree, say $T'$, of height $O(\log n)$ with no factor loss.
Moreover, if $T$ is a tree from a metric-closure of some graph, then we may assume every internal vertex has degree at least two; hence, the height of the $T'$ can be bounded by $O(\log k)$, where $k$ is the number of leaves of $T$. (We may think of leaves of $T$ as terminals in a DST instance.)

In the case of DST, the optimal tree $T$ is an out-arborescence, and the rotation technique would be difficult. In particular, although the two subtrees $T_{left}$ and $T_{right}$ (so called {\em left} and {\em right} subtrees, respectively) that we obtain from the balanced vertex separator $v$ are both arborescences, we may have an issue with direction. To see this, one of the subtrees, say $T_{left}$ may have $r$ as a root and have $v$ as either a leaf or an internal vertex, while $T_{right}$ has $v$ as a root vertex.
%
Now as we rotate the arborescence to make $v$ a root vertex, the $r\mapsto{v}$-path in the graph will be in a wrong direction. (We are supposed to have a path from $v$ to vertices in $T_{left}$ not the $r\mapsto{v}$-path.)
Hecne, we need to introduce a new root vertex $r'$, which is a copy of $r$, that joins the two arborescences $T_{left}$ and $T_{right}$ so that all the paths are in the right direction.
Let us denote the new tree by $T'$.
It is not hard to see that $T'$ may not exist in the metric-closure of $T$,
deeming all the previous DST algorithms useless.
In addition, even if we have a subgraph, say ${\bf G}$, that contains all the possible such trees $T'$, an optimal out-arborescence $T^*\subseteq {\bf G}$ might not correspond to any out-arborescence in the input graph.

Let us circumvent this problem in a recursive manner.
From here, we will denote an instance of DST consisting of an $n$-vertex directed graph $G$, a root vertex $r$ and a set of terminals $S$ by $I=(G,r,S)$.
%
Let us start by presenting a simple case, where we assume that we know a balanced vertex separator $v$ of the optimal solution and we also know which terminals will be on which parts of the subtrees.
%
Then we can use $v$ to partition the set of terminals $S$ into $S_{left}$ and $S_{right}$.
Thus, we have to solve two subproblems $I_{left}=(G,r,S_{left}\cup\{v\})$ and $I_{right}=(G,r,S_{right})$. We remark that we need to add $v$ to $S_{left}\cup{v}$ because we have to ensure that the solution from the left subproblem $I_{left}$ connects the root $r$ to $v$ (which will be the root of an optimal out-arborescence of $I_{left}$). Otherwise, when we merge the sub-solutions together, it would not be an out-arborescence in the original input graph. It is not hard to see that we can apply the above partitioning operation recursively until we end up with a tree of height $O(\log{k})$, where $k$ here is the number of terminals in the DST instance.

In reality, we face a harder problem because we do not know both the vertex separator of the optimal solution do not know which terminals will appear in the left or in the right subtrees.
%
As such, we have to to iterate over all the possible separators in the input graph $G$.
Let us say, for every vertex $v\in V(G)$, we create two instances of DST, namely, $I_{left}=(G,r,S\cup\{v\})$ and $I_{right}=(G,v,S)$. That is, the left sub-problem has one extra terminal, which we may call {\em label}, while the right sub-problem remains the same DST-instance but with $v$ as a root.
%
Clearly, if we run this recursive procedure up to $O(\log k)$ levels, then we would capture one of the decomposition of the optimal DST solution. So, it suffices to stop the recursion when at the depth $O(\log k)$ even if we do not know which subtree corresponds to the optimum.
%
Consequently, this recursive procedure ends up constructing $O(n^{O(\log k)})$ instances of DST, and each instances may have up to $O(\log k)$ extra terminals (labels). Although we create a lot DST instances, the decision tree of this process only has {\bf height $O(\log k)$}.

We capture the {\em decision tree} of this process by defining the Label-Consistent subtree problem as defined in \Cref{sec:prelim}. In fact, this recursive technique has been known as the {\em branch decomposition}, which allows one to solve many problems on bounded-tree width graphs or trees optimally; however, it is not the case for us as our problem is NP-hard even when the input graph is a tree (because it include the GST problem on trees as a special case).

\subsection{Second Ingredient: Lifting Label-Consistent LP}
\label{sec:overview:lifting-LP}

Now we assume that we already have a reduction from an instance of DST to an instance of LCST on a tree ${\bf T}$ of height $O(\log k)$.

In addition, the extra terminal is add to only one of the subproblems, and when we solve the problem at a deeper level, an instance $I_{\ell}=(G,v,S\cup L\cup\{w\})$ at level $\ell$, where $w$ is the label added at the level $\ell-1$, we have to make sure that all the other labels that is added in all the level ${\ell'}\leq\ell$ that are not in $L$ has been handled by some instances. This is because even if we have a solution $\tau_{\ell}$ of $I_{\ell}$, that connects the vertex $v$ to $w$, the subgraph $\tau_{\ell}$ may not be out-arborescence rooted at $v$. 

As such, we have an issue on how to deal with extra (up to) $O(\log k)$ labels that are added up. A natural way to this type of problem is to make a guarantee to the subinstance $I_{\ell}$ that all the labels beside $w$ have been handled, and this is a condition that we are given to the algorithm that solves $I_{\ell}$. A natural way to give a condition to a subinstance best on a set of previous decision in the decision tree is to apply a hierarchy techniques. Our choice is to invoke $O(\log k)$ round of Sherali-Adam hierarchy to a natural LP-relaxation of the Label-Consistent Subtree problem. The remaining part is merely standard as we can apply a standard Sherali-Adam LP rounding technique as in \cite{Rothvoss11} or \cite{GuptaXXX}.

*** Need to add this part ***

\subsection{Third Ingredient: Reducing the Height Further}
\label{sec:overview:reducing-more}

